Machine Learning Estimation of Heterogeneous Causal Effects: Empirical Monte Carlo Evidence

We investigate the finite sample performance of causal machine learning estimators for heterogeneous causal effects at different aggregation levels. We employ an Empirical Monte Carlo Study that relies on arguably realistic data generation processes (DGPs) based on actual data. We consider 24 different DGPs, eleven different causal machine learning estimators, and three aggregation levels of the estimated effects. In the main DGPs, we allow for selection into treatment based on a rich set of observable covariates. We provide evidence that the estimators can be categorized into three groups. The first group performs consistently well across all DGPs and aggregation levels. These estimators have multiple steps to account for the selection into the treatment and the outcome process. The second group shows competitive performance only for particular DGPs. The third group is clearly outperformed by the other estimators.

==> App/Converge.tex <==
% Table generated by Excel2LaTeX from sheet 'Convergence'
\begin{table}[htbp]
  \centering \scriptsize
  \caption{Convergence speed of MSE}
    \begin{tabular}{lccccccccccccccc}
    \toprule
Random noise:          & \multicolumn{3}{c}{Yes} &       & \multicolumn{3}{c}{No} &       & \multicolumn{3}{c}{Yes} &       & \multicolumn{3}{c}{No} \\
Selection          & \multicolumn{3}{c}{Yes} &       & \multicolumn{3}{c}{Yes} &       & \multicolumn{3}{c}{No} &       & \multicolumn{3}{c}{No} \\
\cmidrule{2-4}\cmidrule{6-8}\cmidrule{10-12}\cmidrule{14-16}          & ITE   & GATE  & ATE   &       & ITE   & GATE  & ATE   &       & ITE   & GATE  & ATE   &       & ITE   & GATE  & ATE \\
    \midrule
          & \multicolumn{15}{c}{ITE0} \\
    \midrule
    \textit{Random Forest:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 0.93  & 0.73  & 0.26  &       & \multicolumn{3}{c}{-} &       & 0.93  & 0.73  & 0.26  &       & \multicolumn{3}{c}{-} \\
    Conditional mean regression & 0.77  & 0.60  & 0.45  &       & 0.75  & 0.59  & 0.45  &       & 0.74  & 0.53  & 0.21  &       & 0.70  & 0.53  & 0.22 \\
    Causal Forest & 0.67  & 0.49  & 0.55  &       & 0.65  & 0.50  & 0.55  &       & 0.64  & 0.28  & 0.22  &       & 0.57  & 0.28  & 0.22 \\
    Causal Forest with local centering & 0.65  & 0.32  & 0.28  &       & 0.60  & 0.32  & 0.28  &       & 0.64  & 0.28  & 0.22  &       & 0.58  & 0.28  & 0.22 \\
    MOM IPW & 0.61  & 0.26  & 0.39  &       & 0.57  & 0.26  & 0.39  &       & 0.65  & 0.30  & 0.22  &       & 0.60  & 0.29  & 0.22 \\
    MOM DR & 0.66  & 0.35  & 0.32  &       & 0.58  & 0.35  & 0.31  &       & 0.62  & 0.27  & 0.22  &       & 0.52  & 0.27  & 0.22 \\
    \textit{Lasso:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 0.94  & 0.44  & 0.26  &       & \multicolumn{3}{c}{-} &       & 0.94  & 0.39  & 0.26  &       & \multicolumn{3}{c}{-} \\
    Conditional mean regression & 0.57  & 0.44  & 0.40  &       & 0.54  & 0.44  & 0.39  &       & 0.56  & 0.39  & 0.22  &       & 0.54  & 0.39  & 0.22 \\
    MOM IPW & 0.47  & 0.37  & 0.34  &       & 0.44  & 0.37  & 0.34  &       & 0.32  & 0.22  & 0.22  &       & 0.21  & 0.22  & 0.22 \\
    MOM DR & 0.05  & 0.01  & 0.00  &       & 0.01  & 0.01  & 0.01  &       & 0.39  & 0.22  & 0.21  &       & 0.21  & 0.21  & 0.22 \\
    MCM   & 0.43  & 0.35  & 0.30  &       & 0.42  & 0.36  & 0.31  &       & 0.32  & 0.22  & 0.22  &       & 0.21  & 0.22  & 0.22 \\
    MCM with efficiency augmentation & 0.37  & 0.26  & 0.27  &       & 0.23  & 0.26  & 0.27  &       & 0.40  & 0.23  & 0.22  &       & 0.22  & 0.22  & 0.22 \\
    R-learning & 0.38  & 0.27  & 0.28  &       & 0.23  & 0.26  & 0.27  &       & 0.40  & 0.23  & 0.22  &       & 0.23  & 0.22  & 0.22 \\
    \midrule
          & \multicolumn{15}{c}{ITE1} \\
    \midrule
    \textit{Random Forest:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 1.15  & 0.74  & 0.23  &       & 0.94  & 0.63  & 0.21  &       & 1.15  & 0.74  & 0.23  &       & 0.94  & 0.63  & 0.21 \\
    Conditional mean regression & 0.81  & 0.64  & 0.54  &       & 0.78  & 0.67  & 0.63  &       & 0.79  & 0.57  & 0.22  &       & 0.75  & 0.59  & 0.22 \\
    Causal Forest & 0.73  & 0.59  & 0.64  &       & 0.72  & 0.67  & 0.74  &       & 0.71  & 0.35  & 0.22  &       & 0.69  & 0.46  & 0.22 \\
    Causal Forest with local centering & 0.72  & 0.39  & 0.33  &       & 0.69  & 0.48  & 0.39  &       & 0.71  & 0.35  & 0.22  &       & 0.69  & 0.47  & 0.23 \\
    MOM IPW & 0.69  & 0.26  & 0.41  &       & 0.64  & 0.39  & 0.41  &       & 0.71  & 0.37  & 0.22  &       & 0.70  & 0.51  & 0.23 \\
    MOM DR & 0.74  & 0.39  & 0.33  &       & 0.70  & 0.47  & 0.36  &       & 0.70  & 0.36  & 0.22  &       & 0.69  & 0.51  & 0.22 \\
    \textit{Lasso:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 1.01  & 0.60  & 0.24  &       & 0.79  & 0.42  & 0.25  &       & 1.01  & 0.60  & 0.24  &       & 0.79  & 0.42  & 0.25 \\
    Conditional mean regression & 0.61  & 0.45  & 0.43  &       & 0.57  & 0.42  & 0.41  &       & 0.63  & 0.41  & 0.22  &       & 0.57  & 0.37  & 0.22 \\
    MOM IPW & 0.53  & 0.38  & 0.36  &       & 0.50  & 0.40  & 0.38  &       & 0.43  & 0.33  & 0.23  &       & 0.47  & 0.56  & 0.22 \\
    MOM DR & 0.07  & 0.01  & 0.01  &       & 0.08  & 0.05  & 0.01  &       & 0.52  & 0.34  & 0.22  &       & 0.56  & 0.55  & 0.22 \\
    MCM   & 0.49  & 0.32  & 0.30  &       & 0.47  & 0.36  & 0.31  &       & 0.45  & 0.33  & 0.22  &       & 0.48  & 0.57  & 0.22 \\
    MCM with efficiency augmentation & 0.52  & 0.34  & 0.28  &       & 0.54  & 0.49  & 0.29  &       & 0.54  & 0.35  & 0.22  &       & 0.58  & 0.57  & 0.22 \\
    R-learning & 0.54  & 0.36  & 0.31  &       & 0.56  & 0.51  & 0.34  &       & 0.54  & 0.36  & 0.23  &       & 0.57  & 0.57  & 0.22 \\
    \midrule
          & \multicolumn{15}{c}{ITE2} \\
    \midrule
    \textit{Random Forest:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 1.09  & 0.69  & 0.28  &       & 0.97  & 0.70  & 0.25  &       & 1.09  & 0.69  & 0.28  &       & 0.97  & 0.70  & 0.25 \\
    Conditional mean regression & 0.90  & 0.70  & 0.66  &       & 0.93  & 0.58  & 0.50  &       & 0.89  & 0.64  & 0.24  &       & 0.95  & 0.39  & 0.21 \\
    Causal Forest & 0.86  & 0.66  & 0.75  &       & 0.84  & 0.65  & 0.72  &       & 0.84  & 0.53  & 0.24  &       & 0.98  & 0.31  & 0.21 \\
    Causal Forest with local centering & 0.85  & 0.52  & 0.43  &       & 1.01  & 0.38  & 0.35  &       & 0.84  & 0.53  & 0.24  &       & 0.98  & 0.32  & 0.22 \\
    MOM IPW & 0.84  & 0.56  & 0.44  &       & 0.80  & 0.55  & 0.40  &       & 0.83  & 0.56  & 0.24  &       & 0.86  & 0.56  & 0.22 \\
    MOM DR & 0.87  & 0.52  & 0.38  &       & 1.06  & 0.45  & 0.34  &       & 0.84  & 0.57  & 0.23  &       & 1.06  & 0.35  & 0.21 \\
    \textit{Lasso:} &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Infeasible & 0.97  & 0.62  & 0.32  &       & 0.83  & 0.45  & 0.23  &       & 0.97  & 0.62  & 0.32  &       & 0.83  & 0.45  & 0.23 \\
    Conditional mean regression & 0.76  & 0.45  & 0.44  &       & 0.67  & 0.35  & 0.31  &       & 0.77  & 0.41  & 0.23  &       & 0.69  & 0.34  & 0.22 \\
    MOM IPW & 0.71  & 0.45  & 0.41  &       & 0.64  & 0.38  & 0.41  &       & 0.68  & 0.59  & 0.24  &       & 0.75  & 0.51  & 0.22 \\
    MOM DR & 0.49  & 0.12  & 0.02  &       & 0.29  & 0.09  & 0.01  &       & 0.76  & 0.59  & 0.23  &       & 0.84  & 0.34  & 0.21 \\
    MCM   & 0.69  & 0.41  & 0.29  &       & 0.70  & 0.61  & 0.33  &       & 0.68  & 0.62  & 0.22  &       & 0.71  & 0.69  & 0.21 \\
    MCM with efficiency augmentation & 0.76  & 0.55  & 0.32  &       & 0.81  & 0.40  & 0.28  &       & 0.76  & 0.60  & 0.24  &       & 0.87  & 0.35  & 0.22 \\
    R-learning & 0.78  & 0.56  & 0.38  &       & 0.83  & 0.42  & 0.30  &       & 0.76  & 0.61  & 0.24  &       & 0.87  & 0.35  & 0.22 \\
    \bottomrule
    \end{tabular}%
   \label{tab:converge}
\end{table}%
